Theoretical band-gap bounds and coupling sensitivity for a periodic medium with branching resonators

Elastic metamaterials may exhibit band gaps at wavelengths far exceeding feature sizes. This is attributed to local resonances of embedded or branching substructures. In branched configurations, such as a pillared plate, waves propagating in the base medium-e.g., the plate portion-experience attenuation at band-gap frequencies. Considering a simplified lumped-parameter model for a branched medium, we present a theoretical treatment for a periodic unit cell comprising a base mass-spring chain with a multi-degree-of-freedom, mono-coupled branch. Bloch's theorem is applied, combined with a sub-structuring approach where the resonating branch is modelled separately and condensed into its effective dynamic stiffness. Thus, the treatment is generally applicable to an arbitrary branch regardless of its size and properties. We provide an analysis-with guiding graphical illustrations-that yields an identification of fundamental bounds for the band-gap edges as dictated by the dynamical characteristics of the branch. Analytical sensitivity functions are also derived for the dependence of these bounds on the degree of coupling between the base and the branch. The sensitivity analysis reveals further novel findings including the role of the frequency derivative of the branch dynamic stiffness in providing a direct relation between the band-gap edge locations and variation in the coupling parameters-the mass and stiffness ratios between the base chain and the branch root. In additional analysis, sub-Bragg bounds of an exact model comprising a one-dimensional (1D) continuous base-modelled as a rod-and a discrete branch are derived and shown to be tighter than those of the all-discrete model. Finally, the applicability of the derived bounds and sensitivity functions are shown to be valid for a corresponding full 2D finite-element model of a pillared waveguide admitting out-of-plane shear waves.

==> tmp.tex <==
....
....

\end{abstract}

%%Graphical abstract
\begin{graphicalabstract}
%\includegraphics{grabs}
\end{graphicalabstract}

%%Research highlights
\begin{highlights}
\item Research highlight 1
\item Research highlight 2
\end{highlights}

\begin{keyword}
%% keywords here, in the form: keyword \sep keyword
....
....

